Code Review Comprehension: Reviewing Strategies Seen Through Code Comprehension Theories

Despite the popularity and importance of modern code review, the understanding of the cognitive processes that enable reviewers to analyze code and provide meaningful feedback is lacking. To address this gap, we observed and interviewed ten experienced reviewers while they performed 25 code reviews from their review queue. Since comprehending code changes is essential to perform code review and the primary challenge for reviewers, we focused our analysis on this cognitive process. Using Letovsky's model of code comprehension, we performed a theory-driven thematic analysis to investigate how reviewers apply code comprehension to navigate changes and provide feedback. Our findings confirm that code comprehension is fundamental to code review. We extend Letovsky's model to propose the Code Review Comprehension Model and demonstrate that code review, like code comprehension, relies on opportunistic strategies. These strategies typically begin with a context-building phase, followed by code inspection involving code reading, testing, and discussion management. To interpret and evaluate the proposed change, reviewers construct a mental model of the change as an extension of their understanding of the overall software system and contrast mental representations of expected and ideal solutions against the actual implementation. Based on our findings, we discuss how review tools and practices can better support reviewers in employing their strategies and in forming understanding. Data and material: https://doi.org/10.5281/zenodo.14748996

==> sections/graveyard.tex <==
Reviewers load information from the Information Sources (see \ref{sec:information_sources}), predominantly the PR itself, in connection to their Knowledge Base (\ref{sec:knowledge_base}) to construct the Mental Model of the code change and its extensions (\ref{sec:mental_model}). Reviewers use their own knowledge to detect issues in the PR and find further knowledge sharing opportunities that enable them to evaluate the code change and provide constructive feedback in the review comments. Reviewers knowledge and mental model of the PR enable them to create new artifacts - the review comments - that become information source for the author and other reviewers.

However, working memory is a limited resource~\cite{paas2003cognitive} and the cognitive load that a task poses on the cognitive system can deplete the available capacity, thus leading to cognitive overload and poor performance~\cite{paas2003cognitive, matthews2019stress}. Therefore, this capacity should be used efficiently.

TESTING PAPER:
- Why is testing important
- Dependency on human labor and challenges
- Literature on testing is plenty, but devs are the ones that need to put it all together and come up with relevant test cases
- What they did
- COntributions - framework, a set of actionable guidelines

there are also more structured and formal techniques available to support reviewers in performing the reviews such as checklist-based reading or a range of scenario-based reading techniques~\cite{baum2019cognitive, ciolkowski2003software}.

Review participantys should seek out the explanations from each other to improve their understanding~\cite{widyasari2023explaining}.
